VISCR: Intuitive & Conflict-free Automation for Securing the Dynamic Consumer IoT Infrastructures

Consumer IoT is characterized by heterogeneous devices with diverse functionality and programming interfaces. This lack of homogeneity makes the integration and security management of IoT infrastructures a daunting task for users and administrators. In this paper, we introduce VISCR, a Vendor-Independent policy Specification and Conflict Resolution engine that enables conflict-free policy specification and enforcement in IoT environments. VISCR converts the topology of the IoT infrastructure into a tree-based abstraction and translates existing policies from heterogeneous vendor-specific programming languages such as Groovy-based SmartThings, OpenHAB, IFTTT-based templates, and MUD-based profiles into a vendor-independent graph-based specification. Using the two, VISCR can automatically detect rouge policies, conflicts, and bugs for coherent automation. Upon detection, VISCR infers new policies and proposes them to users as alternatives to existing policies for fine-tuning and conflict-free enforcement. We evaluated VISCR using a dataset of 907 IoT apps, programmed using heterogeneous automation specifications in a simulated smart-building IoT infrastructure. In our experiments, among 907 IoT apps, VISCR exposed 342 of IoT apps as exhibiting one or more violations. VISCR detected 100% of violations reported by existing state-of-the-art tool, while detecting new types of violations in an additional 266 apps. In terms of performance, VISCR can generate 400 abstraction trees (used in specifying policies) with 100K leaf nodes in <1.2sec. In our experiments, VISCR took 80.7 seconds to analyze our infrastructure of 907 apps; a 14.2X reduction compared to the state-of-the-art. After the initial analysis, VISCR is capable of adopting new policies in sub-second latency to handle changes.

==> background.tex <==
We use the term IoT Infrastructure in this paper to refer to networks of Internet-enabled embedded devices with sensing and actuation capabilities that specifically represents {\em Consumer IoT} (e.g., smart home, smart campus, smart city and enterprise IoT networks).



\vspace{3pt}
 \noindent \textbf{Policy \& Automation Frameworks}: {\em Automation} in the context of an IoT infrastructure refers to the mechanism by which different IoT devices are programmed to automatically communicate with each other for carrying out specific task in the cyber-physical environment. Similarly, {\em IoT policies} refer to sets of rules that govern the working of IoT devices in dynamic network environments, while securing the IoT infrastructure and preserving the privacy and safety of its users. For simplicity, we use the terms {\em IoT policies}, {\em IoT automation rules}, {\em IoT apps} and {\em IoT programs} interchangeably in our paper. Similarly, the {\em smartphone app} or {\em mobile app} provides necessary graphical user interface by which devices belonging to specific vendor can be configured or programmed. 

The following two types of policies are required for effectively automating the IoT infrastructures and governing the communication among its devices: %($i$) Trigger- \& Action-based automation rules, and ($ii$) ACL-based (Access Control List) policies.



\begin{packeditemize}

% \vspace{3 pt}
% \noindent 
\item
\textbf{Trigger- \& Action-based Rules}: These rules allow the administrator to specify policies on a set of devices that perform some action in response to an event. Example of programming specification mechanisms used for these type of policies includes SmartThings Groovy-based rules~\cite{groovy_smartthingsapps}, OpenHAB-based rules~\cite{openhab}, IFTTT-based applets~\cite{decouple_ifttt}, and Apple HomeKit~\cite{apple_iot_homekit_swift}.% (graph-based representation with \secintent is shown in Figure \ref{figure:dynamic_trigger_action_policy_graph}). 
% Examples of such policies are illustrated in Figure \ref{figure:dynamic_trigger_action_policy_graph}. 


% \vspace{3pt}
% \noindent 
\item
\textbf{ACL-based Policies}: The ACL-based policies restrict the type of communication the IoT devices are permitted, during normal and abnormal states, within the IoT ecosystem. Example of policy specification mechanisms used for IoT infrastructures include MUD-based profiles~\cite{mud_spec} and traditional IP tuple-based filtering rules. %(graph-based representation with \secintent is shown in Figure \ref{figure:static_dynamic_acl_policies_graph}). 
% Examples of ACL-based policies are shown in Figure \ref{figure:static_dynamic_acl_policies_graph}.

\end{packeditemize}

 

==> background_intro.tex <==
%In this section, we describe the background details and highlight the key challenges that motivate the need for development of \secintent for existing consumer and enterprise IoT infrastructures.

==> grammar_files.tex <==
\begin{figure}[h!]
\includegraphics[width=1.0\linewidth,height=2in]{images/dummy.png}
\caption{\small Grammar snippet (.g4) files for Groovy-based SmartThings \& OpenHAB-based IoT apps.}\label{figure:groovy_grammer_g4_openhab}
\end{figure}


% \begin{figure}[h!]
% \includegraphics[width=1.0\linewidth,height=2in]{images/dummy.png}
% \caption{\small Sample Grammar .g4 file for OpenHAB-based IoT automation specification.}\label{figure:openhab_grammar_g4}
% \end{figure}

% \begin{figure}[h!]
% \includegraphics[width=1.0\linewidth,height=2in]{images/dummy.png}
% \caption{\small Sample Grammar .g4 file for IFTTT-based IoT automation specification.}\label{figure:ifttt_grammar_g4}
% \end{figure}

% \begin{figure}[h!]
% \includegraphics[width=1.0\linewidth,height=2in]{images/dummy.png}
% \caption{\small Sample Grammar .g4 file for MUD-based IoT policy specification.}\label{figure:mud_grammar_g4}
% \end{figure}

==> implementation_testbed_eval.tex <==
% In this section, we discuss the prototype implementation of \secintent and test-bed details followed by evaluations of abstraction, specification and composition engines. %\blue{We highlight the details of our user-study in evaluating the expressibility and efficacy of \secintentnospace.}

==> inference.tex <==





==> introduction_old_may_15_2019_1PM.tex <==
The swift adoption of the Internet of Things (IoT) has led to a significant explosion in the number of devices that are being rapidly integrated into consumer IoT infrastructures (e.g., ``smart homes'', ``smart campus'', and ``smart cities'') ~\cite{gartner-future-smart-home,gartner_2020}. % \blue{\sout{Gartner Inc. predicts that by 2022, a single ``smart home'' is likely to have over 500 connected devices~\cite{gartner-future-smart-home}, while a ``smart campus'' or ``smart city'' may have millions of devices attached to its ecosystem~\cite{gartner_2020}.}}
This rise in popularity of IoT devices also raise several new challenges to consumer IoT infrastructures: 


\begin{packeditemize}

\item [$(1)$]
{\it Policy Expressibility}:  Most IoT device vendors support web and mobile-based apps that allow users and administrators to program their IoT infrastructures.  However, directly capturing the high level automation (or policy) intent of IoT administrators, using these vendor-specific apps, is a challenging task as it requires administrators to manually decompose their high-level intents into device-specific rules prior to installation onto IoT infrastructures for deployment. In general, such manual processes are prone to errors and leave gaps in automation that make IoT infrastructures vulnerable~\cite{iotsmartapp_vulnerabilities}. Hence, IoT users and administrators rely on IoT automation frameworks and specification languages to fulfill their complex automation needs~\cite{openhab,apple_iot_homekit,groovy_smartthingsapps,mud_spec}. However, vendor-support limitations, imposed by each of these automation frameworks, often forces IoT administrators to deploy and use multiple automation frameworks for effectively programming their IoT infrastructure~\cite{dzone_automation_frameworks}. Hence, intuitively capturing the automation rules and policies in a vendor-agnostic manner is a critical challenge.


\item [$(2)$]
{\it Coherent Automation}: A variety of automation frameworks and  policy specification languages are used in programming the consumer IoT infrastructures. For example, Samsung SmartThings~\cite{groovy_smartthingsapps} uses Groovy-based automation rule specification language, Apple HomeKit~\cite{apple_iot_homekit_swift} uses Swift-based programming specifications, and tens of other custom programming specifications are used today for automation~\cite{dzone_automation_frameworks}. Realizing {\it coherent} automation within an IoT ecosystem, i.e., free of conflicts, errors and bugs in the presence of heterogeneous specification mechanisms is another important challenge.

\item [$(3)$]
{\it Conflict-free Enforcement}: Consumer IoT infrastructures are programmed by multiple administrators having complex {\it roles} and varying levels of {\it skill}, which includes novice smart-home users (e.g., parents, kids), smart-campus `or' smart-city administrators (e.g., HVAC admins, fire-safety admins). %The multi-administrative environments that uses heterogeneous programming frameworks, realizing {\it conflict-free} automation is a tedious process, which requires IoT administrators to collaborate with each other (i.e., to chart out their policies) for manually resolving the conflicts that might arise in automating their IoT ecosystems. 
Contemplating {\it conflict-free} automation in such multi-administrative environments is a tedious process, which requires IoT administrators to collaborate with each other for charting out their automation rules and policies, and manually resolve the conflicts that might arise among their automation and policy intents. For example, a fire-safety administrator's automation intent to open the windows and turn OFF HVAC in case of temperature crossing a threshold could conflict with building administrator's automation rule to keep the windows and doors closed after 10PM or during week-ends for safety and security concerns.

\end{packeditemize}


\vspace{2pt}
%Therefore, the lack of {\it coherent} and {\it intuitive} automation frameworks leaves IoT infrastructures vulnerable and prone to errors. 
Recent studies independently underscore the need for new access control and policy frameworks to address specifically the security goals of IoT ecosystem~\cite{rethink_acls_iot,soteria,celikiotguard}. These proposed solutions are designed to identify violations in IoT device ecosystems with {\it homogeneous} programming specifications, which does not apply to contemporary consumer IoT deployments that commonly involve devices using diverse vendor-specific APIs and heterogeneous programming specifications. Furthermore, existing tools either rely on model checking for static analysis of IoT automation programs to detect the conflicts \lq or\rq require IoT automation code to be instrumented for detecting run-time violations~\cite{celikiotguard}. In addition, there is a spectrum of automation bugs and conflicts that could go undetected. For example,  {\it gap in automation} due to lack of expertise, {\it rogue policies} on infrastructures that the user does not control, violations that might arise due to loops among automation rules, and other potential run-time conflicts (\S \ref{sec:composition_security_analysis}).

The implication is that specifying each isolated dynamic automation use case correctly requires substantial user effort. Thus, coherently specifying policies for complex deployments, with multiple use cases, programmed to work with hundreds of devices, even within a small-scale IoT infrastructures such as smart homes is an onerous task that involves careful consideration of all potential conflicts and violations.  To holistically address the various challenges, we propose a new intent-based automation framework called ``\secintentnospace'' that provides the following capabilities:

% \begin{packeditemize}

% \item
{\it Vendor-independent (VI) Graph-based specification}: For effectively handling heterogeneity, the automation rules and policies specified by IoT users and administrators using heterogeneous programming specification languages inside an IoT infrastructure are translated into vendor-independent graph-based specifications. For example, in our framework we translate the IoT automation programs specified using groovy-based programs for smarthings, OpenHAB-based rules, MUD-profiles and IFTTT-based applets into vendor-independent graph-based specifications (\S \ref{sec:vi_spec}). \secintent also allows multiple policy administrators of an IoT infrastructure to directly and succinctly capture their dynamic automation use-cases and policy intents in a vendor-independent manner using simple graph-based abstractions (\S \ref{sec:abstractions_graph-based-specification}).
% For effectively accommodating {\it heterogeneous} automation frameworks and specification languages, we propose \visenospace, a Vendor-Independent Specification \& IoT app analysis Engine that translates automation rules and policies programmed using heterogeneous specification languages (e.g., Groovy for smartThings, OpenHAB-based rules, MUD profiles and IFTTT-based applets) into vendor-independent graph-based specifications (\S \ref{sec:vi_spec}). \vise analysis IoT apps to evaluate the {\it code sanity} and detect bugs present in the code (\S \ref{sec:code_sanity_analysis}). Our \secintent framework also allows administrators of an IoT infrastructure to succinctly capture their dynamic automation use cases and policy intents in a vendor-independent manner with {\it simple graph-based policy specification} using {\it tree-based infrastructure abstractions} (\S \ref{sec:abstractions_graph-based-specification}). 



% \item
{\it Graph-based Composition \& Security Analysis}: The vendor-independent graph-based policy specifications captured using the approaches discussed in \S \ref{sec:vi_spec} and \S \ref{sec:abstractions_graph-based-specification} are composed together for conflicts and analyzed for bugs among these policies. With the graph-based composition \secintent identifies the bugs that could otherwise go undetected using existing model checking-based tools~\cite{soteria,celikiotguard}. For example, our tool detects wide range of bugs and conflicts among automation rules (\S \ref{sec:composition_security_analysis}) such as: ($a$) compile-time conflicts, ($b$) gap in the automation, ($c$) conflicts due to loops among automation rules, ($d$) code sanity bugs, ($e$) access violations, and ($f$) rogue policies. 


% \item
{\it Conflict-free Enforcement \& Policy Inference}:
For automatically resolving the conflicts, \secintent supports {\tt PRECEDENCE} operators, while unresolved conflicts are forwarded to appropriate IoT users or administrators for manual resolution. The policy reconciliation and enforcement engine decomposes a composed conflict-free policy graph into a set of device-specific rules for enforcement onto actual devices (e.g., IoT devices, IoT Gateways) as IoT apps and ACLs. In addition, the enforcement engine infers new policy and propose it to IoT users for fine-tuning the existing policies and addressing the security and safety violations that arise among the policies (\S \ref{sec:policy_enforcement}).


% \end{packeditemize}

Our evaluation of \secintent on simulated smart building IoT infrastructure detected a wide range of bugs i.e., $\approx$37.7\% of IoT apps are reported for one or more conflicts and bugs compared to $\approx$8.4\% of static compile-time conflicts detected with existing model checking-based tool~\cite{soteria}. %The overall percentage of conflicts and bugs reported by \secintent estimated upto $\approx$55.9\% of overall IoT apps 
%\blue{with $\approx$10.3\% of the policies has showcased more than one type of policy conflicts or bugs}. 
\secintent is able to identify $\approx$29.3\% of new conflicts and bugs compared to existing tools~\cite{soteria}, resulting in approximately $<$7.8\% false positives or low intense bugs. The resultant conflicts and bugs that are detected by \secintent categorized according to their type are highlighted in Table \ref{table:smart-building-polcy-conflicts} (\S \ref{sec:prototype_evaluations}).
%\secintent has proactively detected $\approx$11.8\% of potential run-time conflicts. 
%\red{\sout{\secintent was able to propose \red{$\approx$XY\%} of new policies to resolve the conflicts through {\it inference} for resolving the conflicts (Section \ref{sec:prototype_evaluations}).}}

\noindent In summary, our paper makes the following key contributions:

\begin{packeditemize}


\item
Design of \visenospace, a Vendor-Independent Specification \& code analysis Engine that translates automation rules and policies specified using heterogeneous programming specification languages into vendor-independent graph-based policies. Carries out security analysis to evaluate the {\it code sanity} and detect bugs present in the code. We develop intuitive policy specification mechanism using tree-based abstractions that allows users to directly capture the vendor-independent graph-based policies for automation and policy specification (Section \ref{sec:vi_spec_code_analysis}).

\item
Development of a composition engine that detects various bugs and conflicts that arise among the vendor-independent graph-based policies and resolve the conflicts that arise among the policies and automation rules using {\tt PRECEDENCE} operation for conflict-free enforcement. We developed techniques to automatically infer new policies for proposing to user for fine-tuning the existing rules (\S \ref{sec:composition_security_analysis}).

\item
Evaluation of \secintent using $\approx$900 IoT apps (i.e., both vetted and unvetted), in a simulated smart building infrastructure with real world automation use-cases, conflicts and bugs reported by actual IoT users and administrators in their real IoT infrastructures and comparison with existing techniques (\S \ref{sec:prototype_evaluations}).

\end{packeditemize}





==> motivation.tex <==
\subsection{Motivation}\label{sec:motivation}

Today, consumer IoT infrastructures (e.g., smart home, smart campus, smart city) pose diversity along multiple dimensions: ($i$) \blue{heterogeneity} in their device-types, functional capabilities, vendor-types, and ($ii$) heterogeneity in automation programming specifications they use. Such heterogeneity makes programming the IoT infrastructure a challenging task. In addition, these consumer IoT infrastructures are {\it multi-administrative domains} i.e., manged by multiple users or administrators with different roles and responsibilities, which further complicates automation of IoT infrastructures leading to conflicts and errors. \blue{For example, the smart home automation rules and policies are specified by the members of the family (e.g., parents, kids, guests), while smart campus and enterprise IoT infrastructures are managed by different types of IoT administrators such as HVAC, fire-safety, utilities \& energy, and infrastructure (or building) administrators.} Therefore, the {\it heterogeneity} among IoT devices and the lack of a unified policy-specification mechanism to cater the needs of multiple administrators of consumer IoT infrastructures forces IoT administrators to independently develop automation policies and uses offline mechanisms (e.g., via email) to exchange their policies. Such independently-developed policies, which are often exchanged offline are configured on to each of the IoT devices by manually inspecting each of the rules for conflicts. 

Today, a variety of automation frameworks, and automation specification languages are supported by vendors for automating the IoT infrastructures, which includes SmartThings using groovy-based specification~\cite{groovy_smartthingsapps}, OpenHAB~\cite{openhab}, Apple IoT HomeKit~\cite{apple_iot_homekit}, IFTTT-based templates~\cite{decouple_ifttt}, MUD-based profiles~\cite{mud_spec}. But, these policy frameworks are limited along following key dimensions: ($i$) Intuitive policy specification, and ($ii$) Conflict detection \& resolution. Next, we discuss about each of these limitations with necessary motivational scenarios that highlight the need for a {\em unified}, and {\em vendor-independent} policy-specification mechanism, and efficient conflict detection and resolution mechanisms to handle {\em dynamic} IoT policies.

\subsection{Intuitive  Policy Specification}
Currently, policy intents of an IoT administrator are implemented using discrete automation rules configured onto each device using the corresponding vendor's API and automation specification languages~\cite{groovy_smartthingsapps,openhab,mud_spec,samsung_ifttt}. \blue{These vendor-specific APIs and automation specification languages allow IoT users and administrators to independently capture their automation rules and policies specific to their infrastructure's security, safety, and privacy needs. Today, the consumer IoT ecosystem lacks effective mechanisms for reconciling policy intents from various users. }
\red{<To Be Added>}


\begin{figure}[t!]
\includegraphics[width=1.0\linewidth,height=1.5in]{images/dummy.png}
\caption{\small Code Sanity issues commonly seen in existing IoT Apps: Improper conditional block closures, Empty If/Else blocks, Undefined or Unreferenced variables and structures.}\label{figure:code_sanity_undefined_unfererenced}
\end{figure}

\red{@Vasu: Discuss about Heterogeneity \& Multi-administrative domains.}



\red{@Vasu: Illustrate the need for graph-based policies and graph-based composition. Why the existing composition SAT-based techniques fall short in performance and types of bugs they detect with some example?}


\red{@Vasu: Illustrate need for VI models. Here, it should capture the what challenges does the heterogeneity and multi-admin domain brings with illustration examples from related work. 1) No isolation leading to rogue policies, 2) No vendor-independent representation leading or not able to handle multiple admins could lead to conflicts (example, talk about almond, iotguard, )}



\red{@Vasu: Consider following examples: ($i$) A parent's intent to access all the smart home video feeds at any instance of time could be restricted by the kid to provide access to his/her bedroom's video feeds after 10PM. ($ii$) Consider for examples policies P1 and P2 in Table \ref{table:policy-intents}. In case of fire-event, when the video feed is shared with fire-safety administrators, the inactivity timer could kick in and turn off the video sharing leads to safety violations. A major concern with such policies is that they are activated in response to an event received from one or more sensors.} 

\blue{Aforementioned examples demonstrate the need for collaboration across administrators of these IoT infrastructures for charting out their policies and manually resolve the conflicts that arise among their policies before enforcing them onto IoT infrastructure.}








\subsection{Conflict Detection \& Resolution}\label{motive:conflict_detect_resolve}

Lack of efficient conflict detection mechanisms that can seamlessly compose the automation use-cases and policies specified using different \red{\sout{automation}} specification languages leaves these infrastructures vulnerable to multiple security, safety, and privacy threats. Recent studies have also demonstrated that major vulnerabilities in the IoT infrastructure are commonly due to simple human errors and lack of expertise \red{\sout{(or skills)}} in policy configuration~\cite{iot_vulnerability1,iot_vulnerability2,openhab_missing_quotes,openhab_missing_if_braces}.



\begin{figure}[t!]
\includegraphics[width=1.0\linewidth,height=1.5in]{images/dummy.png}
\caption{Illustration of conflicts, violations and bugs in consumer IoT Infrastructures. \red{@Vasu: Illustrate with example all the types of bugs and illustrate need for our approach and highlight how they are rather difficult to be detected using existing techniques in Figure 2}}\label{figure:conflicts_violations_bugs_motivation}
\end{figure}



\vspace{2pt}
\noindent {\em Static Policy Conflict}: Consider two policies P3 and P7 with conflicting actions with respect to opening doors (Table \ref{table:policy-intents}). In case of a fire alarm after 10 P.M., (both policies P3 and P4 are activated) the current IoT automation keeps the door locked due to policy P3, preventing users from leaving and fire-safety officers from entering. \red{Proactively detecting such conflicting actions resulting in safety violations is a challenging task.} 


\vspace{3pt}
\noindent {\em Dynamic Policy Violation}: As illustrated in Figure \ref{figure:motivation_conflict}, policies P1 and P2 results in runtime violation. When video feed is shared with fire-safety staff, the video feed is interrupted by the camera's idle-time event which turns OFF the camera. Such violations are difficult to be detected and resolved in run-time as the asynchronous inactivity counter is triggered, which depends on environmental conditions, (i.e., time and motion sensing). Also, automatically detecting and resolving such conflicts in existing IoT frameworks is complicated by device heterogeneity and reliance on complex syntax-based policy-specification mechanisms. 



\red{@Vasu: Illustrate sequence in example 2, how sequence in which the events occur could create different types of violations. P1: >9PM when light turned ON, Close Windows; P2: When Blinds are closed automatically close windows; P3: In case of fire-incident open windows. The sequence in which they occur makes them acceptable or not i.e., either leads to violation or acceptable automation. Similarly, the video-feed sharing and fire-incident. Make these scenarios as two small diagrams in the single column.}

Therefore, a fundamental requirement for any IoT-based policy framework is to effectively handle the dynamic characteristics of IoT infrastructure and adapt to such dynamic changes and enforce new set of policies by proactively detect and resolve new conflicts that arise at runtime.  


==> precedence_reconciliation.tex <==
Precedence operators are used to resolve conflicts among competing policies specified at different levels. {\it Administrator-level precedence} evaluation is based on the scope of authority of the policy author. For example, a campus-level administrator in a smart campus may be granted precedence over a building administrator; %or an IoT-security admin policies could be given precedence over building administrators utilities  \& energy policies.
{\it Action-level precedence} allows for explicit prioritization in action invocation. For example, for IoT traffic's ACL-based policies, Drop $>$ Allow $>$ Quarantine $>$ Redirect can be used as the precedence hierarchy. Similarly, in the case of trigger-action-based policies, when the smoke detector is in {\tt \small fire-alarm} state, the action turn OFF heating is given higher precedence than turn ON heating. {\it Custom precedence} enables policy attributes (e.g., {\tt \small user}, {\tt \small device type}, {\tt \small device state}) to be associated with precedence.  

When two policies (P1 and P2) conflict, the nodes and edges of the policies are decomposed into the {\it set of subset nodes that requires the least number of edges to represent conflict-free policies} (for optimizing the number of rules required for enforcement).  Based on precedence, the overlapping nodes that result in conflict are removed and the edge specific to the policy with highest precedence is retained.

